Self-critiquing models for assisting human evaluators

We fine-tune large language models to write natural language critiques (natural language critical comments) using behavioral cloning. On a topic-based summarization task, critiques written by our models help humans find flaws in summaries that they would have otherwise missed. Our models help find naturally occurring flaws in both model and human written summaries, and intentional flaws in summaries written by humans to be deliberately misleading. We study scaling properties of critiquing with both topic-based summarization and synthetic tasks. Larger models write more helpful critiques, and on most tasks, are better at self-critiquing, despite having harder-to-critique outputs. Larger models can also integrate their own self-critiques as feedback, refining their own summaries into better ones. Finally, we motivate and introduce a framework for comparing critiquing ability to generation and discrimination ability. Our measurements suggest that even large models may still have relevant knowledge they cannot or do not articulate as critiques. These results are a proof of concept for using AI-assisted human feedback to scale the supervision of machine learning systems to tasks that are difficult for humans to evaluate directly. We release our training datasets, as well as samples from our critique assistance experiments.

==> sections/apdx.extra_disc.tex <==
Figure \ref{fig:discriminator_scaling_winrate} showed discriminator scaling for judging between answers to the same questions.  We also looked at discriminator scaling "across questions":  we look at Spearman correlation, Pearson correlation and ROC AUC.   Figure \ref{fig:discriminator_scaling_score} shows "across questions" scaling.



\begin{figure}
\centering
\begin{subfigure}[t]{.49\textwidth}
  \includegraphics[width=\linewidth]{plots/gdgap_scoring_global.png}
  % \captionof{figure}{Even if not filtering for critiqueable}
   \captionof{figure}{
Without assistance:  critiqueability labels come from humans finding critiques with no assistance
   }
   \label{fig:discriminator_scaling_score_noassist}
   \end{subfigure}
\hspace*{\fill} 
\begin{subfigure}[t]{.49\textwidth}
  \includegraphics[width=\linewidth]{plots/gdgap_assisted.png}
  \captionof{figure}{
  With assistance: critiqueability labels come from humans that also see critiques from the discriminator model.
  % This somewhat contradicts the results from Figure \ref{fig:discriminator_scaling_winrate}.  % Although more capable models get better at recognizing good answers, their ability to generate answers appears to roughly cancel that out.
  }
  \label{fig:discriminator_scaling_score_assisted}

\end{subfigure} 


  \caption{  
Discriminator scaling.  Unlike Figure \ref{fig:discriminator_scaling_winrate}, we assess discrimination across answers to different questions.  We score by critiqueability according to the model, on answers generated from the same model, and compare to the binary human critiqueability labels, using various scoring functions for discriminators.  
}
  
    \label{fig:discriminator_scaling_score}

\end{figure}


We can also look at the absolute quality of responses as a function of model size and amount of optimization against the critiqueability discriminator (Figure \ref{fig:discriminator_scaling_boN_likert}).  Unlike what we saw with win rate, the Likert differences between best-of-N and best-of-1 are diminishing with model size.


\begin{figure}
\centering
  \includegraphics[width=\linewidth]{plots/gdboNLikert.png}
  % \captionof{figure}{Even if not filtering for critiqueable}
   \captionof{figure}{
   Performance of best-of-N against the critiqueability discriminator.  Gains from best-of-N do not clearly improve with model size, but this is also true with best-of-N against the human critiqueability label itself.  Note that the effect of best-of-N against the human labeler is exaggerated due to selecting directly against the selections of the same human.  We make no attempt to control for this (e.g. with a second labeler), as it is not our main interest.
   }
   \label{fig:discriminator_scaling_boN_likert}

\end{figure}


TODO organize
\begin{figure}
\centering
  \includegraphics[width=\linewidth]{plots/synthetic_disc.png}
  % \captionof{figure}{Even if not filtering for critiqueable}
   \captionof{figure}{
   Synthetic tasks discriminator (critiqueability) ability
   }
   \label{fig:synthetic_discriminator}

\end{figure}




